Opetopic algebras III: Presheaf models of homotopy-coherent opetopic algebras

For $\Lambda$ the category of free opetopic algebras, we construct a model structure \emph{\`a la Cisinski} on the category of presheaves over $\Lambda$, and show that is is equivalent to opetopic complete Segal spaces. This generalizes the results of Joyal and Tierney in the simplicial case, and of Cisinski and Moerdijk in the planar dendroidal case.

==> macros.tex <==
%
% macros.tex
% v2.2 2019/02/15
%

\makeatletter

% ------------------------------------------------------------------------------
% AUTOMATA
% ------------------------------------------------------------------------------

\newcategory{\Auto}{}{A}{uto}

\newcommand{\acc}{\mathrm{acc}}
\newcommand{\init}{\mathrm{init}}
\DeclareMathOperator{\triv}{triv}

% ------------------------------------------------------------------------------
% CATEGORIES
% ------------------------------------------------------------------------------

\newcategory{\Ctx}{}{C}{tx} % Category of contexts (syntaxtic category)

% ------------------------------------------------------------------------------
% General
% ------------------------------------------------------------------------------

\DeclareMathOperator{\eqdef}{\coloneq}
\DeclareMathOperator{\equivdef}{:\!\equiv}
\DeclareMathOperator{\hash}{\#}
\newcommand{\condition}[1]{\textbf{\upshape{(#1)}}}

% ------------------------------------------------------------------------------
% OPETOPES
% ------------------------------------------------------------------------------

\newcategory{\PshO}{}{\widehat{\bbOO}}{}
\newcategory{\FinO}{}{F}{in\PshO}

\newcommand{\opetope}[1]{\left\lbrace\begin{matrix*}[l]#1\end{matrix*}\right.}
\newcommand{\degenopetope}[1]{\left\lbrace \!\! \opetope{#1} \right.}
\newcommand{\sep}{\leftarrow}

\newcommand{\optZero}{\filledlozenge}
\newcommand{\optOne}{\filledsquare}
\newcommand{\optInt}[1]{\mathbf{#1}}

\newcommand{\namedcoding}[1]{\left\lBrack #1 \right\rBrack^!}
\newcommand{\polycoding}[1]{\left\lBrack #1 \right\rBrack^{\mathrm{poly}}}
\newcommand{\unnamedcoding}[1]{{\left\lBrack #1 \right\rBrack^?}}

\newcommand{\optPolyFun}{\frakZZ}

\newcommand{\shape}[1]{#1^\natural}

\newcommand{\universal}{\filledtriangleright}

% ------------------------------------------------------------------------------
% POLYGRAPHS
% ------------------------------------------------------------------------------

\newcategory{\Pol}{}{P}{ol}
\newcommand{\MTO}{\triangledown}
\newcommand{\PolMTO}{\Pol^\MTO}

% ------------------------------------------------------------------------------
% POLYNOMIAL FUNCTORS
% ------------------------------------------------------------------------------

\newcategory{\PolyEnd}{}{P}{oly{\catEE}nd}
\newcategory{\PolyMnd}{}{P}{oly{\catMM}nd}
\newcategory{\Tree}{}{T}{ree}

\newcommand{\polynomialfunctor}[7]{
    \begin{tikzpicture}
        \matrix (m) [matrix of math nodes,
        row sep = 2 em,
        column sep = 2 em,
        text height = 1.5ex,
        text depth = 0.25ex,
        ampersand replacement = \&] {
            \displaystyle{#1} \&
            \displaystyle{#2} \&
            \displaystyle{#3} \&
            \displaystyle{#4} \\
        };
        \path[->]
            (m-1-2) edge node [above] {$#5$} (m-1-1)
            (m-1-2) edge node [above] {$#6$} (m-1-3)
            (m-1-3) edge node [above] {$#7$} (m-1-4);
    \end{tikzpicture}
}

% ------------------------------------------------------------------------------
% PROOFTREES
% ------------------------------------------------------------------------------

\newenvironment{prooftree*}{\leavevmode\hbox\bgroup}{\DisplayProof\egroup}

% ------------------------------------------------------------------------------
% TIKZ
% ------------------------------------------------------------------------------

\newcommand{\DDownarrow}{
    \mathrel{
        \begin{tikz} [baseline=-3pt, rotate=-90]
            \draw [shorten >= 0pt, shorten <= 0pt]
                (0, 3pt)  -- ++(1.5ex, 0)
                (0, 1pt)  -- ++(1.5ex+1pt, 0)
                (0, -1pt) -- ++(1.5ex + 1pt, 0)
                (0, -3pt) -- ++(1.5ex, 0)
                (1.5ex - 1pt, 5pt)
                    to [in = 135, out = -75] (1.5ex + 2pt, 0)
                    to [out = -135, in = 75] (1.5ex - 1pt, -5pt);
		\end{tikz}
	}
}

% This command alows to import parts of tikz files. The ``main'' tag is imported
% by default, and other tags can be specified in 3rd argument as a comma
% separated list (with NO SPACES!). 2nd argument is file name, expected to be in
% ``tikz/'' subdir. 1st argument in is optional, and is the tikz scale factor
\usepackage{catchfilebetweentags}
\newcommand{\tikzinput}[3][1]{
	\begin{tikzpicture}
        \tikzset{scale = #1}
		\ExecuteMetaData[tikz/#2.tikz]{main}
		\@for\tmp:=#3\do{
			\ExecuteMetaData[tikz/#2.tikz]{\tmp}
		}
	\end{tikzpicture}
}


\newcommand{\pullbackcorner}{
    \ar[dr, phantom, "\lrcorner", very near start, shift right = 0ex]
}
\newcommand{\pushoutcorner}{
    \ar[dr, phantom, "\ulcorner", very near end, shift right = 0ex]
}

% ------------------------------------------------------------------------------
% TODO
% ------------------------------------------------------------------------------

%\newcommand{\TODO}[1]{\marginpar{\tiny #1}}

% ------------------------------------------------------------------------------
% TREES
% ------------------------------------------------------------------------------

\newcommand{\itree}[1]{\mathsf{I}_{#1}}
\newcommand{\ytree}[1]{\mathsf{Y}_{#1}}

\newcommand{\leafsymbol}{|}
\newcommand{\nodesymbol}{\bullet}

\DeclareMathOperator{\tree}{tr}
\DeclareMathOperator{\treewithleaf}{tr^{\leafsymbol}}
\DeclareMathOperator{\treewithnode}{tr^{\nodesymbol}}

\newcommand{\underlyingtree}[1]{\left\langle #1 \right\rangle}

\newcommand{\addr}{\&}

\newcommand{\subst}{\operatornamewithlimits{\smallsquare}}
\newcommand{\graft}{\operatornamewithlimits{\circ}}
\newcommand{\grafti}{\operatornamewithlimits{\tilde{\circ}}}
\DeclareMathOperator*{\biggraft}{\bigcircle}

\DeclareMathOperator{\src}{\mathsf{s}}
\DeclareMathOperator{\tgt}{\mathsf{t}}
\DeclareMathOperator{\edg}{\mathsf{e}}

\newcommand{\readdress}{\wp}
\newcommand{\substreaddress}{\chi}

\makeatother

==> tikz/common.tex <==
\usetikzlibrary{calc, decorations.pathmorphing, positioning}

% args: x, y, w, h, label, inner x, innner y
\newenvironment{TIKZZONE}[7]{
\begin{scope} [shift = {(#1, #2)}]
\draw [dotted] (0, 0) node [above right] {\small{\texttt{#5}}} -- (0, #4) -- (#3, #4) -- (#3, 0) -- cycle;
\begin{scope} [shift = {(#6, #7)}]
}{
\end{scope} \end{scope}
}

\tikzset{treeedge/.style = {above, sloped}}
\tikzset{treenode/.style = {circle, minimum size = 2pt, inner sep = 0, draw, fill}}

\newcommand{\blackwhitespoon}{-}
\newcommand{\DDownarrow}{|}
\newcommand{\optInt}[1]{\textbf{#1}}
\newcommand{\optOne}{\rightarrow}
\newcommand{\optZero}{\bullet}
\newcommand{\readdress}{P}
\newcommand{\RRightarrow}{-}
\newcommand{\Rrightarrow}{\equiv\!>}
\newcommand{\smalltriangleright}{>}
\newcommand{\src}{\mathsf{s}}
\newcommand{\system}{\textsc}
\newcommand{\tgt}{\mathsf{t}}
